Spreading and Suppression of Infection Clusters on the Ginibre Continuum Percolation Clusters

Off-lattice SIR models are constructed on continuum percolation clusters defined on the Ginibre point process (GPP) and on the Poisson point process (PPP). The static percolation transitions in the continuum percolation models as well as the infection-spreading transitions in the SIR models, which are regarded as the dynamic percolation transitions, are enhanced in the GPP-based model compared with the PPP-based model. This enhancement is caused by hyperuniformity of the GPP. On the other hand, in the extinction phase of infection on the phase diagram, a wide parameter region is determined in which formation of infection clusters is suppressed in the GPP-based model compared with the PPP-based model. We think that the PPP approximates a disordered configuration of individuals and the GPP does a configuration of citizens adopting a strategy to keep social distancing in a city in order to avoid contagion. The suppression of infection clusters observed in the GPP-based model will prove that such a strategy is effective when the infectivity is relatively small.

==> tex/bibliography.tex <==
%%%%%REFERENCES%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{thebibliography}{99} 
\bibitem{KK21}
Machiko Katori, Makoto Katori, 
Continuum percolation and stochastic epidemic models 
on Poisson and Ginibre point processes. 
{\sf arXiv:2103.08461}

\bibitem{Gilb61}
E. N. Gilbert,
J. Soc. Indust. Appl. Math.
\textbf{9}, 533 (1961)

\bibitem{MR96}
R. Meester and R. Roy,
\textit{Continuum Percolation}
(Cambridge University Press, Cambridge, 1996)

\bibitem{BR06}
B. Bollobas and O. Riordan,
\textit{Percolation}
(Cambridge University Press, Cambridge, 2006)

\bibitem{DVJ03}
D. J. Daley and D. Vere-Jones,
\textit{An Introduction to the Theory of Point Processes},
Vol. i, 2nd ed.
(Springer, New York, 2003)

\bibitem{Gra83}
P. Grassberger,
Math. Biosci.
\textbf{63}, 157 (1983)

\bibitem{MDVZ99}
M. A. Mu\~noz, R. Dickman, A. Vespignani, and S. Zapperi,
Avalanche and spreading exponents in systems 
with absorbing states,  
Phys. Rev. E 
\textbf{59}, 6175 (1999)

\bibitem{dST10}
D. R. de Souza and T. Tom\'e,
Physica A
\textbf{389}, 1142 (2010)

\bibitem{TZ10}
T. Tom\'e and R. M. Ziff,
Phys. Rev. E
\textbf{82}, 051921 (2010)

\bibitem{SMDHB20}
S. Saha, A. Mishra, S. K. Dana, C. Hens, and N. Bairagi, 
Phys. Rev. E
\textbf{102}, 052307 (2020)

\bibitem{SAAMF20}
G. B. M. Santosa, T. F. A. Alvesa, G. A. Alvesb, 
A. Macedo-Filhoc, and R. S. Ferreirad, 
Phys. Lett. A
\textbf{384}, 126063 (2020)

\bibitem{Lig85}
T. Liggett,
\textit{Interacting Particle Systems}
(Springer, New York, 1985). 

\bibitem{Lig99}
T. Liggett,
\textit{Stochastic Interacting Systems:
Contact, Voter and Exclusion Processes}
(Springer, New York, 1999). 

\bibitem{MD99}
J. Marro and R. Dickman,
\textit{Nonequilibrium Phase Transitions
in Lattice Models}
(Cambridge University Press, Cambridge, 1999)

\bibitem{Hin00}
H. Hinrichsen,
Adv. Phys.
\textbf{49}, 815 (2000)

\bibitem{CG85}
J. Cardy and P. Grassberger,
J. Phys. A
\textbf{18}, L267 (1985)

\bibitem{Zif21}
R. M. Ziff,
Physica A
\textbf{568}, 125723 (2021)

\bibitem{Gin65}
J. Ginibre, 
J. Math. Phys.
\textbf{6}, 440 (1965)

\bibitem{Shi06}
T. Shirai,
J. Stat. Phys. 
\textbf{123}, 615 (2006)

\bibitem{HKPV09}
J. Hough, M. Krishnapur, Y. Peres,
B. Vir\'ag,
\textit{Zeros of Gaussian Analytic Functions
and Determinantal Point Processes}
(American Mathematical Society, 
Providence, RI, 2009)

\bibitem{Meh04}
M. L. Mehta, 
\textit{Random Matrices}, 3rd edn
(Elsevier/Academic Press, Amsterdam, 2004) 

\bibitem{For10}
P. J. Forrester, 
\textit{Log-gases and Random Matrices}
(Princeton University Press, Princeton, NJ, 2010)

\bibitem{Kat16}
M. Katori,
\textit{Bessel Processes, Schramm--Loewner Evolution,
and the Dyson model}
(Springer, Singapore, 2016)

\bibitem{Tor18}
S. Torquato, 
Phys. Rep. 
\textbf{745}, 1 (2018)

\bibitem{MKS21}
T. Matsui, M. Katori, and T. Shirai, 
J. Phys. A: Math. Theor. 
\textbf{54}, 165201 (2021)

\bibitem{GL17}
Ghosh, S., Lebowitz, J. L., 2017,
Fluctuations, large deviations and rigidity 
in hyperuniform systems:
A brief survey,
Indian J. Pure Appl. Math. 
\textbf{48}, 609--631

\bibitem{BY13}
B. B{\l}aszcyszyn and D. Yogeshwarany, 
Elect. J. Probab.
\textbf{18}, no.72, 1 (2013)

\bibitem{BY14}
B. B{\l}aszcyszyn and D. Yogeshwarany, 
Adv. Appl. Prob. (SGSA)
\textbf{46}, 1 (2014)

\bibitem{GKP16}
S. Ghosh, M. Krishnapur, and Y. Peres, 
Ann. Probab. 
\textbf{44}, 3357 (2016)

\bibitem{SA92}
D. Stauffer and A. Aharony,
\textit{Introduction to Percolation Theory}
(Taylor \& Francis, London, 1992)

\bibitem{MM12}
S. Mertens and C. Moore,
Phys. Rev. E 
\textbf{86}, 061109 (2012)

\bibitem{QT99}
J. Quintanilla and S. Torquato,
J. Chem. Phys.
\textbf{111}, 5947 (1999)

\bibitem{QTZ00}
J. Quintanilla, S. Torquato, and R. M. Ziff,
J. Phys. A: Math. Gen. 
\textbf{33}, L399 (2000)

\bibitem{NZ01}
M. E. J. Newman and R. M. Ziff,
Phys. Rev. E
\textbf{64}, 016706 (2001)

\bibitem{QZ07}
J. A. Quintanilla and R. M. Ziff,
Phys. Rev. E
\textbf{76}, 051115 (2007)

\bibitem{Gil76}
D. Gillespie,
J. Comput. Phys.
\textbf{22}, 403 (1976)

\bibitem{Gil77}
D. Gillespie,
J. Phys. Chem.
\textbf{81}, 2340 (1977)

\bibitem{EC20}
R. Erban and S. J. Chapman,
\textit{Stochastic Modeling of Reaction-Diffusion Processes}
(Cambridge University Press, Cambridge, 2020)



\end{thebibliography}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

